Steganography: a class of secure and robust algorithms

This research work presents a new class of non-blind information hiding algorithms that are stego-secure and robust. They are based on some finite domains iterations having the Devaney's topological chaos property. Thanks to a complete formalization of the approach we prove security against watermark-only attacks of a large class of steganographic algorithms. Finally a complete study of robustness is given in frequency DWT and DCT domains.

==> abstract.tex <==
%Chaos-based approaches are frequently proposed
%in information hiding, but without obvious justification. 
%Indeed, the reason why chaos is useful to tackle with discretion, 
%robustness, or security, is rarely elucidated. 
This research work presents a new class of non-blind information hiding
algorithms that are stego-secure and robust.
They are based on some finite domains iterations having the Devaney's 
topological chaos property.
Thanks to a complete formalization of the approach we prove   
security against watermark-only attacks
of a large class of steganographic algorithms.
Finally a complete study of robustness is given in frequency DWT and DCT domains.



==> applications.tex <==
We are then left to provide an u.d. strategy-adapter that is independent
from the cover, an image mode $f_l$ whose iteration
graph $\Gamma(f_l)$ is strongly connected and whose Markov
matrix is doubly stochastic.

First, the $\textit{CIIS}(K,y,\alpha,l)$ strategy adapter (see Section~\ref{sub:wmcoding})
has the required properties:
it does not depend on the cover and the proof that its outputs
are u.d. on $\llbracket 1; l \rrbracket$ 
is left as an exercise for the reader.
In all the experiments parameters $K$ and $\alpha$ are randomly 
chosen in $\rrbracket 0, 1\llbracket$ and $\rrbracket 0, 0.5\llbracket$
respectively.
The number of iteration is set to $4*lm$, where $lm$ is the number of LSCs 
that depends on the domain.  
 
Next,~\cite{bcgr11:ip} has presented an iterative approach to generate image
modes $f_l$ such that $\Gamma(f_l)$ is strongly connected. Among these
maps, it is obvious to check which verifies or not the doubly
stochastic constrain.
For instance, in what follows we consider the mode
$f_l: \Bool^l \rightarrow \Bool^l$ s.t. its $i$th component is
defined by
\begin{equation}
\label{eq:fqq}
{f_l}(x)_i =
\left\{
\begin{array}{l}
\overline{x_i} \textrm{ if $i$ is odd} \\
x_i \oplus x_{i-1} \textrm{ if $i$ is even}
\end{array}
\right.
\end{equation}

Thanks to~\cite[Theorem 2]{bcgr11:ip} we deduce that its iteration graph 
$\Gamma(f_l)$ is strongly connected. 
Next, the Markov chain is stochastic by construction. 

Let us prove that its Markov chain is doubly stochastic by induction on the 
length $l$.
For $l=1$ and $l=2$ the proof is obvious. Let us consider that the 
result is established until $l=2k$ for some $k \in \Nats$.

Let us then firstly prove the doubly stochasticity for $l=2k+1$.
Following notations introduced in~\cite{bcgr11:ip}, 
let  $\Gamma(f_{2k+1})^0$ and $\Gamma(f_{2k+1})^1$ denote
the subgraphs of $\Gamma(f_{2k+1})$ induced by the subset $\Bool^{2k} \times\{0\}$
and $\Bool^{2k} \times\{1\}$ of $\Bool^{2k+1}$ respectively.
$\Gamma(f_{2k+1})^0$ and   $\Gamma(f_{2k+1})^1$ are isomorphic to $\Gamma(f_{2k})$.
Furthermore, these two graphs are linked together only with arcs of the form
$(x_1,\dots,x_{2k},0) \to (x_1,\dots,x_{2k},1)$ and 
$(x_1,\dots,x_{2k},1) \to (x_1,\dots,x_{2k},0)$.
In $\Gamma(f_{2k+1})$ the number of arcs whose extremity is $(x_1,\dots,x_{2k},0)$
is  the same than the number of arcs whose extremity is $(x_1,\dots,x_{2k})$ 
augmented with 1, and similarly for $(x_1,\dots,x_{2k},1)$.
By induction hypothesis, the Markov chain associated to $\Gamma(f_{2k})$ is doubly stochastic. All the vertices $(x_1,\dots,x_{2k})$ have thus the same number of 
ingoing arcs and the proof is established for $l$ is $2k+1$.

Let us then  prove the doubly stochasticity for $l=2k+2$.
The map $f_l$ is defined by 
$f_l(x)= (\overline{x_1},x_2 \oplus x_{1},\dots,\overline{x_{2k+1}},x_{2k+2} \oplus x_{2k+1})$.
With previously defined  notations, let us focus on 
$\Gamma(f_{2k+2})^0$ and   $\Gamma(f_{2k+2})^1$ which are isomorphic to $\Gamma(f_{2k+1})$. 
Among configurations of $\Bool^{2k+2}$, only four suffixes of length 2 can be
obviously observed, namely, $00$, $10$, $11$ and $01$.
Since 
$f_{2k+2}(\dots,0,0)_{2k+2}=0$, $f_{2k+2}(\dots,1,0)_{2k+2}=1$, 
$f_{2k+2}(\dots,1,1)_{2k+2}=0$, and $f_{2k+2}(\dots,0,1)_{2k+2}=1$, the number of 
arcs whose extremity is 
\begin{itemize}
\item $(x_1,\dots,x_{2k},0,0)$
 is the same than the one whose extremity is $(x_1,\dots,x_{2k},0)$ in $\Gamma(f_{2k+1})$ augmented with 1 (loop over configurations $(x_1,\dots,x_{2k},0,0)$);
\item $(x_1,\dots,x_{2k},1,0)$
 is the same than the one whose extremity is $(x_1,\dots,x_{2k},0)$ in $\Gamma(f_{2k+1})$ augmented with 1 (arc from configurations 
$(x_1,\dots,x_{2k},1,1)$ to configurations 
$(x_1,\dots,x_{2k},1,0)$);
\item $(x_1,\dots,x_{2k},0,1)$
 is the same than the one whose extremity is $(x_1,\dots,x_{2k},0)$ in $\Gamma(f_{2k+1})$ augmented with 1 (loop over configurations $(x_1,\dots,x_{2k},0,1)$);
\item $(x_1,\dots,x_{2k},1,1)$
 is the same than the one whose extremity is $(x_1,\dots,x_{2k},1)$ in $\Gamma(f_{2k+1})$ augmented with 1 (arc from configurations 
$(x_1,\dots,x_{2k},1,0)$ to configurations 
$(x_1,\dots,x_{2k},1,1)$).
\end{itemize}
Thus all the vertices $(x_1,\dots,x_{2k})$ have  the same number of 
ingoing arcs and the proof is established for $l=2k+2$.




==> attacks.tex <==



As far as we know, Cachin~\cite{Cachin2004}
produces the first fundamental work in information hiding security:
in the context of steganography, the attempt of an attacker to distinguish 
between an innocent image and a stego-content is viewed as an hypothesis 
testing problem.
Mittelholzer~\cite{Mittelholzer99} next proposed the first theoretical 
framework for analyzing the security of a watermarking scheme.
Clarification between  robustness and security 
and classifications of watermarking attacks
have been firstly presented by Kalker~\cite{Kalker2001}.
This work has been deepened by Furon \emph{et al.}~\cite{Furon2002}, who have translated Kerckhoffs' principle (Alice and Bob shall only rely on some previously shared secret for privacy), from cryptography to data hiding. 

More recently~\cite{Cayre2005,Perez06} classified the information hiding  
attacks into categories, according to the type of information the attacker (Eve)
has access to:
\begin{itemize}
\item in Watermarked Only Attack (WOA) she only knows embedded contents $z$;
\item in Known Message Attack (KMA) she knows pairs $(z,y)$ of embedded
  contents and corresponding messages;
\item in Known Original Attack (KOA) she knows several pairs $(z,x)$ 
  of embedded contents and their corresponding original versions;
\item in Constant-Message Attack (CMA) she observes several embedded
  contents $z^1$,\ldots,$z^k$ and only knows that the unknown 
  hidden message $y$ is the same in all contents.
\end{itemize}

To the best of our knowledge, 
KMA, KOA, and CMA have not already been studied
due to the lack of theoretical framework.
In the opposite, security of data hiding against WOA can be evaluated,
by using a probabilistic approach recalled below.





==> instantia.tex <==

% The \emph{CIDS} strategy-adapter 
% (\emph{Chaotic Iterations with Dependent Strategy}) 
% with parameters $(N,X) \in \mathds{N}\times \mathds{B}^\mathds{N}$ 
% is the function which 
% associates to any $n\in \mathds{N}$ 
% the sequence $\left(S^t\right)^{t \in \mathds{N}}$ defined as follows:
% \begin{itemize}
%  \item $\forall t \leqslant N$, if $t \leqslant n$ and $X^t = 1$, then $S^t=t$, else $S^t=1$.
%  \item $\forall t > N, S^t = 0$.
% \end{itemize}








% \begin{definition}%[CIIS strategy-adapter]

The \emph{CIIS} strategy-adapter
(\emph{Chaotic Iterations with Independent Strategy}) with parameters 
$(K,M,\alpha,N) \in [0,1]\times [0,1] \times ]0; 0,5[ \times \mathds{N}$
is the function which associates to any  $n \in \Nats$ the sequence
$(S^t)^{t \in \mathds{N}}$ defined by:
 \begin{itemize}
 \item $K^0 = M \oplus K$: $K^0$ is the real number whose binary decomposition is obtained by achieving the bitwise exclusive 
   between the binary decompositions of $M$ and of  $K$;
 \item $\forall t \leqslant N, K^{t+1} = F(K^t,\alpha)$;
 \item $\forall t \leqslant N, S^t = \left \lfloor n \times K^t \right \rfloor + 1$;
 \item $\forall t > N, S^t = 0$.
 \end{itemize}
where $F$ is 
piecewise linear chaotic map~\cite{Shujun1,Arroyo08}, 
recalled in what follows:

\begin{definition}[Piecewise linear chaotic map]
 \label{def:fonction chaotique linéaire par morceaux}
Let $\alpha \in ]0; 0,5[$ be a control parameter. 
The \emph{piecewise linear chaotic map} is the map $F$
defined by: 
 $$
 F(t,\alpha) = \left\{
 \begin{array}{cl} 
 \dfrac{t}{\alpha} & t \in [0; \alpha],\\ 
 \dfrac{t-\alpha}{\frac{1}{2}-\alpha} & t \in [\alpha;\frac{1}{2}],\\ 
 F(1-t,\alpha) & t \in [\frac{1}{2}; 1].\\ 
 \end{array}
 \right. 
 $$
 \end{definition}







==> qualitativeandquantitative.tex <==

Let us firstly recall two fundamental tools taken from the mathematical theory of chaos.

\begin{definition}[Expansivity]
A function $f$ is said to be \emph{expansive} if $
\exists \varepsilon >0,\forall x\neq y,\exists n\in \mathds{N}%
,d(f^{n}(x),f^{n}(y))\geqslant \varepsilon .$
\end{definition}

\begin{definition}[Topological mixing]
A discrete dynamical system is said to be topologically mixing
if and only if, for any couple of disjoint open set $U, V \neq \varnothing$,
$n_0 \in \mathds{N}$ can be found so that $\forall n \geqslant n_0, f^n(U) \cap
V \neq \varnothing$.
\end{definition}

We have proven in \cite{gfb10:ip} that chaotic iterations are expansive and topologically mixing when using the vectorial negation $f_0$. These topological properties are inherited by \emph{dhCI dissimulation} we presented here and lead to improve its unpredictability. In particular, any ignorance or error on the private embedding key are magnified until being equal to the constant of expansivity. We will now investigate the consequences of being chaotic, as defined by Devaney. 

First of all, the transitivity property implies the indecomposability of the system:

\begin{definition}
A dynamical system $\left( \mathcal{X}, f\right)$ is indecomposable if it is not the union of two closed sets $A, B \subset \mathcal{X}$ such that $f(A) \subset A, f(B) \subset B$.
\end{definition}

Thus it is impossible to reduce the set of the watermarked images generated by \emph{dhCI dissimulation}, in order to simplify its complexity, when $Gamma_f$ is strongly connected. 
Moreover, it is possible to show that, under this hypothesis, \emph{dhCI dissimulation} is strongly transitive:

\begin{definition}
A dynamical system $\left( \mathcal{X}, f\right)$ is strongly transitive if $\forall x,y \in \mathcal{X},$ $\forall r > 0,$ $\exists z \in \mathcal{X},$ $d(z,x) \leqslant r \Rightarrow$ $\exists n \in \mathds{N}^*,$ $f^n(z)=y$.
\end{definition}

In other words, for all $x,y \in \mathcal{X}$, it is possible to find a point $z$ in the neighborhood of $x$ such that an iterate $f^n(z)$ is $y$. Indeed, this result has been established during the proof of the transitivity presented in~\cite{guyeux09}. Among other things, the strong transitivity property leads to the fact that without the knowledge of the initial inputs of \emph{dhCI dissimulation}, all of the outputs are possible. Additionally, no point of the output space can be discarded when studying this scheme: it is intrinsically complicated and it cannot be decomposed or simplified.

Finally, this dissimulation algorithm possess the instability property:

\begin{definition}
A dynamical system $\left( \mathcal{X}, f\right)$ is unstable if for all $x \in \mathcal{X}$, the orbit $\gamma_x:n \in \mathds{N} \longmapsto f^n(x)$ is unstable, that is: $\exists \varepsilon > 0,$ $\forall \delta > 0,$ $\exists y \in \mathcal{X},$ $\exists n \in \mathds{N},$ $d(x,y) < \delta$ and $d\left(\gamma_x(n), \gamma_y(n)\right) \geqslant \varepsilon.$
\end{definition}

This property, which is implied by the sensitive dependence to the initial condition, leads to the fact that in all of the neighborhoods of any $x$, there are points that are separated from $x$ under iterations of the algorithm. We thus can claim that the behavior of \emph{dhCI dissimulation} is unstable when $\Gamma_f$ is strongly connected.




==> robustness.tex <==
Previous sections have formalized frequential domains embeddings and
has focused on the negation mode and $f_l$ defined in Equ.~(\ref{eq:fqq}).
In the robustness given in this continuation, {dwt}(neg), 
{dwt}(fl), {dct}(neg), {dct}(fl) 
respectively stand for the DWT and DCT embedding 
with the negation mode and with this instantiated mode.
 
For each experiment, a set of 50 images is randomly extracted 
from the database taken from the BOSS contest~\cite{Boss10}. 
Each cover is a $512\times 512$ grayscale digital image and the watermark $y$ 
is given in Fig~\ref{(b) Watermark}. 
Testing the robustness of the approach is achieved by successively applying
on watermarked images attacks like cropping, compression, and geometric 
transformations.
Differences between 
$\hat{y}$ and $\varphi_m(z)$ are 
computed. Behind a given threshold rate, the image is said to be watermarked.  
Finally, discussion on metric quality of the approach is given in 
Sect.~\ref{sub:roc}.

 


Robustness of the approach is  evaluated by
applying different percentage of cropping: from 1\% to 81\%.
Results are presented in Fig.~\ref{Fig:atck:dec}. Fig.~\ref{Fig:atq:dec:img}
gives the cropped image 
where 36\% of the image is removed.
Fig.~\ref{Fig:atq:dec:curves} presents effects of such an attack.
From this experiment, one can conclude that all embeddings have similar 
behaviors.
All the percentage differences are so far less than 50\% 
(which is the mean random error) and thus robustness is established.



\begin{figure}[ht]
  \centering
  % \subfigure[Cropped Image.]{\includegraphics[width=0.24\textwidth]
  %   {5007_dec_307.png}\label{Fig:atq:dec:img}}\hspace{2cm}
  \subfigure[Cropped Image.]{\includegraphics[width=0.24\textwidth]
    {5007_dec_307.eps}\label{Fig:atq:dec:img}}\hspace{2cm}
  \subfigure[Cropping Effect]{
%\includegraphics[width=0.5\textwidth]{atq-dec.pdf}\label{Fig:atq:dec:curves}}
\includegraphics[width=0.5\textwidth]{atq-dec.eps}\label{Fig:atq:dec:curves}}
\caption{Cropping Results}
\label{Fig:atck:dec}
\end{figure}


\subsubsection{Robustness against compression}

Robustness against compression is addressed
by studying both JPEG  and JPEG 2000 image compressions.
Results are respectively presented in Fig.~\ref{Fig:atq:jpg:curves}
and Fig.~\ref{Fig:atq:jp2:curves}.
Without surprise, DCT embedding which is based on DCT 
(as JPEG compression algorithm is) is  more 
adapted to JPEG compression than DWT embedding.
Furthermore, we have a similar behavior for the JPEG 2000 compression algorithm, which is based on wavelet encoding: DWT embedding naturally outperforms
DCT one in that case.  


\begin{figure}[ht]
  \centering
  \subfigure[JPEG Effect]{
%\includegraphics[width=0.45\textwidth]{atq-jpg.pdf}\label{Fig:atq:jpg:curves}}
\includegraphics[width=0.45\textwidth]{atq-jpg.eps}\label{Fig:atq:jpg:curves}}
  \subfigure[JPEG 2000 Effect]{
%\includegraphics[width=0.45\textwidth]{atq-jp2.pdf}\label{Fig:atq:jp2:curves}}
\includegraphics[width=0.45\textwidth]{atq-jp2.eps}\label{Fig:atq:jp2:curves}}
\caption{Compression Results}
\label{Fig:atck:comp}
\end{figure}



\subsubsection{Robustness against Contrast and Sharpness Attack}
Contrast and Sharpness adjustment belong to the the classical set of 
filtering image attacks.
Results of such attacks are presented in 
Fig.~\ref{Fig:atq:fil} where 
Fig.~\ref{Fig:atq:cont:curve} and Fig.~\ref{Fig:atq:sh:curve} summarize 
effects of contrast and sharpness adjustment respectively. 


\begin{figure}[ht]
  \centering
  \subfigure[Contrast Effect]{
%\includegraphics[width=0.45\textwidth]{atq-contrast.pdf}\label{Fig:atq:cont:curve}}
\includegraphics[width=0.45\textwidth]{atq-contrast.eps}\label{Fig:atq:cont:curve}}
  \subfigure[Sharpness Effect]{
%\includegraphics[width=0.45\textwidth]{atq-flou.pdf}\label{Fig:atq:sh:curve}}
\includegraphics[width=0.45\textwidth]{atq-flou.eps}\label{Fig:atq:sh:curve}}
\caption{Filtering Results}
\label{Fig:atq:fil}
\end{figure}

\subsubsection{Robustness against Geometric Transformation}
Among geometric transformations, we focus on  
rotations, \textit{i.e.}, when two opposite rotations 
of angle $\theta$ are successively applied around the center of the image.
In these geometric transformations,  angles range from 2 to 20 
degrees.  
Results are presented in Fig.~\ref{Fig:atq:rot}: Fig.~\ref{Fig:atq:rot:img}
gives the image of a rotation of 20 degrees whereas
Fig.~\ref{Fig:atq:rot:curve} presents effects of such an attack.
It is not a surprise that results are better for DCT embeddings: this approach
is based on cosine as rotation is. 



\begin{figure}[ht]
  \centering
  \subfigure[20 degrees Rotation Image]{
%    \includegraphics[width=0.25\textwidth]{5007_rot_10.png}\label{Fig:atq:rot:img}}
    \includegraphics[width=0.25\textwidth]{5007_rot_10.eps}\label{Fig:atq:rot:img}}

  \subfigure[Rotation Effect]{
%\includegraphics[width=0.45\textwidth]{atq-rot.pdf}\label{Fig:atq:rot:curve}}
\includegraphics[width=0.45\textwidth]{atq-rot.eps}\label{Fig:atq:rot:curve}}

\caption{Rotation Attack Results}
\label{Fig:atq:rot}
\end{figure}

\subsection{Evaluation of the  Embeddings}\label{sub:roc}
We are then left to set a convenient threshold that is accurate to 
determine whether an image is watermarked or not.
Starting from a set of 100 images selected among the Boss image Panel,
we compute the following three sets: 
the one with all the watermarked images $W$,
the one with all successively watermarked and attacked images $\textit{WA}$,
and the one with only the attacked images $A$.
Notice that the 100 attacks for each images 
are selected among these detailed previously.


For each threshold $t \in \llbracket 0,55 \rrbracket$ and a given image 
$x \in \textit{WA} \cup A$, 
differences on DCT are computed. The image is said to be watermarked
if these differences are less than the threshold. 
In the positive case and if $x$ really belongs to 
$\textit{WA}$ it is a True Positive (TP) case.  
In the negative case but if $x$ belongs to 
$\textit{WA}$ it is a False Negative (FN) case.  
In the positive case but if $x$  belongs to 
$\textit{A}$, it is a False Positive (FP) case.  
Finally, in the negative case and if $x$ belongs to
$\textit{A}$, it is a True Negative (TN).  
The True (resp. False) Positive Rate  (TPR) (resp. FPR) is thus computed 
by dividing the number of TP (resp. FP) by 100.

\begin{figure}[ht]
\begin{center}
%\includegraphics[width=7cm]{ROC.pdf}
\includegraphics[width=7cm]{ROC.eps}
\end{center}
\caption{ROC Curves for DWT or DCT Embeddings}\label{fig:roc:dwt}
\end{figure}

The Figure~\ref{fig:roc:dwt} is the Receiver Operating Characteristic (ROC) 
curve. 
For the DWT, it shows that best results are obtained when the threshold 
is 45\% for the dedicated function (corresponding to the point (0.01, 0.88))
and  46\% for the negation function (corresponding to the point (0.04, 0.85)).
It allows to conclude that each time LSCs differences between
a watermarked image and another given image  $i'$ are less than 45\%, we can claim that 
$i'$ is an attacked version of the original watermarked content.
For the two DCT embeddings, best results are obtained when the threshold 
is 44\% (corresponding to the points (0.05, 0.18) and (0.05, 0.28)).

Let us then give some confidence intervals for all the evaluated attacks. The
approach is resistant to:
\begin{itemize}
\item all the croppings where percentage is less than 85;
\item compressions where quality ratio is greater 
  than 82 with DWT embedding and 
  where quality ratio is greater than 67 with DCT one;
\item contrast when strengthening belongs to $[0.76,1.2]$ 
(resp. $[0.96,1.05]$)  in DWT (resp. in DCT) embedding;
\item all the rotation attacks with DCT embedding and a rotation where
angle is less than 13 degrees with DWT one.
\end{itemize}


==> stegosecurity.tex <==


In the Simmons' prisoner problem~\cite{Simmons83}, Alice and Bob are in jail and
they want to,  possibly, devise an escape plan by  exchanging hidden messages in
innocent-looking  cover contents.  These  messages  are to  be  conveyed to  one
another by a common warden named Eve, who eavesdrops all contents and can choose
to interrupt the communication if they appear to be stego-contents.

Stego-security,  defined in  this well-known  context, is  the  highest security
class in Watermark-Only  Attack setup, which occurs when Eve  has only access to
several marked contents~\cite{Cayre2008}.


Let $\mathds{K}$ be the set of embedding keys, $p(X)$ the probabilistic model of
$N_0$ initial  host contents,  and $p(Y|K)$ the  probabilistic model  of $N_0$
marked contents s.t. each host  content has  been marked
with the same key $K$ and the same embedding function.

\begin{definition}[Stego-Security~\cite{Cayre2008}]
\label{Def:Stego-security}  The embedding  function  is \emph{stego-secure}
if  $\forall K \in \mathds{K}, p(Y|K)=p(X)$ is established.
\end{definition}





%Let $\mathds{K}$ be the set of embedding keys, $p(X)$ the probabilistic model of
%$N_0$ initial  host contents,  and $p(Y|K)$ the  probabilistic model  of $N_0$
%marked contents s.t. each host  content has  been marked
%with the same key $K$ and the same embedding function.

%\begin{definition}[Stego-Security]
%\label{Def:Stego-security}  The embedding  function  is \emph{stego-secure}
%if  $\forall K \in \mathds{K}, p(Y|K)=p(X)$ is established.
%\end{definition}

 Stego-security  states that  the knowledge  of  $K$ does  not help  to make  the
 difference  between $p(X)$ and  $p(Y)$.  This  definition implies  the following
 property:
 $$p(Y|K_1)= \cdots = p(Y|K_{N_k})=p(Y)=p(X)$$ 
 This property is equivalent to  a zero Kullback-Leibler divergence, which is the
 accepted definition of the "perfect secrecy" in steganography~\cite{Cachin2004}.


\subsection{The negation mode is stego-secure}
To make this article self-contained, this section recalls theorems and proofs of stego-security for negation mode published in~\cite{gfb10:ip}.

\begin{proposition} \emph{dhCI dissimulation}  of Definition \ref{def:dhCI} with
negation mode and  CIIS strategy-adapter is stego-secure, whereas  it is not the
case when using CIDS strategy-adapter.
\end{proposition}


\begin{proof}   On   the    one   hand,   let   us   suppose    that   $X   \sim
\mathbf{U}\left(\mathbb{B}^n\right)$  when  using  \linebreak CIIS$(K,\_,\_,l)$.
We  prove  by  a
mathematical   induction   that   $\forall    t   \in   \mathds{N},   X^t   \sim
\mathbf{U}\left(\mathbb{B}^n\right)$.

The     base     case     is     immediate,     as     $X^0     =     X     \sim
\mathbf{U}\left(\mathbb{B}^n\right)$. Let us now suppose that the statement $X^t
\sim  \mathbf{U}\left(\mathbb{B}^n\right)$  holds  until for  some $t$. 
Let  $e  \in
\mathbb{B}^n$   and   \linebreak   $\mathbf{B}_k=(0,\cdots,0,1,0,\cdots,0)   \in
\mathbb{B}^n$ (the digit $1$ is in position $k$).

So    
$P\left(X^{t+1}=e\right)=\sum_{k=1}^n
P\left(X^t=e\oplus\mathbf{B}_k,S^t=k\right)$ where  
$\oplus$ is again the bitwise exclusive or. 
These  two events are  independent when
using CIIS strategy-adapter 
(contrary to CIDS, CIIS is not built by using $X$),
 thus:
$$P\left(X^{t+1}=e\right)=\sum_{k=1}^n
P\left(X^t=e\oplus\mathbf{B}_k\right) \times  P\left(S^t=k\right).$$ 

According to the
inductive    hypothesis:   $P\left(X^{n+1}=e\right)=\frac{1}{2^n}   \sum_{k=1}^n
P\left(S^t=k\right)$.  The set  of events $\left \{ S^t=k \right  \}$ for $k \in
\llbracket  1;n \rrbracket$  is  a partition  of  the universe  of possible,  so
$\sum_{k=1}^n                  P\left(S^t=k\right)=1$.                  Finally,
$P\left(X^{t+1}=e\right)=\frac{1}{2^n}$,   which    leads   to   $X^{t+1}   \sim
\mathbf{U}\left(\mathbb{B}^n\right)$.   This  result  is  true  for all  $t  \in
\mathds{N}$ and then for $t=l$.

Since $P(Y|K)$ is $P(X^l)$ that is proven to be equal to $P(X)$,
we thus  have established that, 
$$\forall K  \in [0;1], P(Y|K)=P(X^{l})=P(X).$$ 
So   dhCI   dissimulation   with   CIIS
strategy-adapter is stego-secure.

On  the  other  hand,  due  to  the  definition  of  CIDS,  we  have  \linebreak
$P(Y=(1,1,\cdots,1)|K)=0$. 
%\JFC{Pourquoi? Justifier davantage là ou dans la def de CIDS}
So   there  is   no  uniform  repartition   for  the stego-contents $Y|K$.
\end{proof}



To sum up, Alice  and Bob can counteract Eve's attacks in  WOA setup, when using
dhCI dissimulation with  CIIS strategy-adapter.  To our best  knowledge, this is
the second time an information hiding scheme has been proven to be stego-secure:
the   former  was   the  spread-spectrum   technique  in   natural  marking
configuration with $\eta$ parameter equal to 1 \cite{Cayre2008}.





\subsection{A new class of $\varepsilon$-stego-secure schemes}

Let us prove that,
\begin{theorem}\label{th:stego}
Let $\epsilon$ be positive,
$l$ be any size of LSCs, 
$X   \sim \mathbf{U}\left(\mathbb{B}^l\right)$,
$f_l$ be an image mode s.t. 
$\Gamma(f_l)$ is strongly connected and 
the Markov matrix associated to $f_l$ 
is doubly stochastic. 
In the instantiated \emph{dhCI dissimulation} algorithm 
with any uniformly distributed (u.d.) strategy-adapter 
that is independent from $X$,  
there exists some positive natural number $q$ s.t.
$|p(X^q)- p(X)| < \epsilon$. 
\end{theorem}


\begin{proof}   
Let $\textit{deci}$ be the bijection between $\Bool^{l}$ and 
$\llbracket 0, 2^l-1 \rrbracket$ that associates the decimal value
of any  binary number in $\Bool^{l}$.
The probability $p(X^t) = (p(X^t= e_0),\dots,p(X^t= e_{2^l-1}))$ for $e_j \in \Bool^{l}$ is thus equal to 
$(p(\textit{deci}(X^t)= 0,\dots,p(\textit{deci}(X^t)= 2^l-1))$ further denoted by $\pi^t$.
Let $i \in \llbracket 0, 2^l -1 \rrbracket$, 
the probability $p(\textit{deci}(X^{t+1})= i)$  is 
\[
 \sum\limits^{2^l-1}_{j=0}  
\sum\limits^{l}_{k=1} 
p(\textit{deci}(X^{t}) = j , S^t = k , i =_k j , f_k(j) = i_k ) 
\]
\noindent 
where $ i =_k j $ is true iff the binary representations of 
$i$ and $j$ may only differ for the  $k$-th element,
and where 
$i_k$ abusively denotes, in this proof, the $k$-th element of the binary representation of 
$i$.

Next, due to the proposition's hypotheses on the strategy,
$p(\textit{deci}(X^t) = j , S^t = k , i =_k j, f_k(j) = i_k )$ is equal to  
$\frac{1}{l}.p(\textit{deci}(X^t) = j ,  i =_k j, f_k(j) = i_k)$.
Finally, since $i =_k j$ and $f_k(j) = i_k$ are constant during the 
iterative process  and thus does not depend on $X^t$, we have 
\[
\pi^{t+1}_i = \sum\limits^{2^l-1}_{j=0}
\pi^t_j.\frac{1}{l}  
\sum\limits^{l}_{k=1} 
p(i =_k j, f_k(j) = i_k ).
\]

Since 
$\frac{1}{l}  
\sum\limits^{l}_{k=1} 
p(i =_k j, f_k(j) = i_k ) 
$ is equal to $M_{ji}$ where  $M$ is the Markov matrix associated to
 $f_l$ we thus have
\[
\pi^{t+1}_i = \sum\limits^{2^l-1}_{j=0}
\pi^t_j. M_{ji} \textrm{ and thus }
\pi^{t+1} = \pi^{t} M.
\]

% The calculus of $p(X^{t+1} = e)$ is thus equal to 
% $\pi^{t+1}_i$. 

First of all, 
since the graph $\Gamma(f)$ is strongly connected,
then for all vertices $i$ and $j$, a path can
be  found to  reach $j$  from $i$  in at  most $2^l$  steps.  
There  exists thus $k_{ij} \in \llbracket 1,  2^l \rrbracket$ s.t.
${M}_{ij}^{k_{ij}}>0$.  
As all the multiples $l \times k_{ij}$ of $k_{ij}$ are such that 
${M}_{ij}^{l\times  k_{ij}}>0$, 
we can  conclude that, if
$k$ is the least common multiple of $\{k_{ij}  \big/ i,j  \in \llbracket 1,  2^l \rrbracket  \}$ thus 
$\forall i,j  \in \llbracket  1, 2^l \rrbracket,  {M}_{ij}^{k}>0$ and thus 
$M$ is a regular stochastic matrix.


Let us now recall the following stochastic matrix theorem:
\begin{theorem}[Stochastic Matrix]
  If $M$ is a regular stochastic matrix, then $M$ 
  has an unique stationary  probability vector $\pi$. Moreover, 
  if $\pi^0$ is any initial probability vector and 
  $\pi^{t+1} = \pi^t.M $ for $t = 0, 1,\dots$ then the Markov chain $\pi^t$
  converges to $\pi$ as $t$ tends to infinity.
\end{theorem}

Thanks to this theorem, $M$ 
has an unique stationary  probability vector $\pi$. 
By hypothesis, since $M$ is doubly stochastic we have 
$(\frac{1}{2^l},\dots,\frac{1}{2^l}) = (\frac{1}{2^l},\dots,\frac{1}{2^l})M$
and thus $\pi =  (\frac{1}{2^l},\dots,\frac{1}{2^l})$.
Due to the matrix theorem, there exists some 
$q$ s.t. 
$|\pi^q- \pi| < \epsilon$
and the proof is established.
Since $p(Y| K)$ is $p(X^q)$ the method is then $\epsilon$-stego-secure
provided the strategy-adapter is uniformly distributed.
 \end{proof}

This section has focused on security with regards to probabilistic behaviors. 
Next section studies it in the perspective of topological ones.


==> wmcoding.tex <==
In what follows, $y$ always stands  
for a digital content we wish to hide into a digital host $x$.


The data hiding scheme presented here does not constrain media to have 
a constant size. It is indeed sufficient to provide a function and a strategy 
that may be  parametrized with the size of the elements to modify. 
The \emph{mode} and the \emph{strategy-adapter} defined below achieve 
this goal.  

\begin{definition}[Mode]
\label{def:mode}
A map $f$, which associates to any $n \in \mathds{N}$ an application 
$f_n : \mathds{B}^n \rightarrow \mathds{B}^n$, is called a \emph{mode}.
\end{definition}




%The data hiding scheme presented here does not constrain media to have 
%a constant size. It is indeed sufficient to provide a function and a strategy 
%that may be  parametrized with the size of the elements to modify. 
%The \emph{mode} and the \emph{strategy-adapter} defined below achieve 
%this goal.  

%\begin{definition}[Mode]
%\label{def:mode}
%A map $f$, which associates to any $n \in \mathds{N}$ an application 
%$f_n : \mathds{B}^n \rightarrow \mathds{B}^n$, is called a \emph{mode}.
%\end{definition}

For instance, the \emph{negation mode} is defined by the map that
assigns to every integer $n \in \mathds{N}^*$ the function 
$${\neg}_n:\mathds{B}^n \to \mathds{B}^n, 
(x_1, \hdots, x_n) \mapsto (\overline{x_1}, \hdots, \overline{x_n}).$$



\begin{definition}[Strategy-Adapter]
  \label{def:strategy-adapter}
  A \emph{strategy-adapter}\index{configuration} is a function $\mathcal{S}$ 
  from $\Nats$ to the set of integer sequences, 
  which associates to $n$ a sequence 
  $S \in  \llbracket 1, n\rrbracket^\mathds{N}$.
\end{definition}

Intuitively, a strategy-adapter aims at generating a strategy 
$(S^t)^{t \in \Nats}$ where each term $S^t$ belongs to 
$\llbracket 1, n \rrbracket$. Moreover it may be parametrized
in order to depend on digital media to embed. 

For instance, let us define the  \emph{Chaotic Iterations with Independent Strategy}
(\emph{CIIS}) strategy-adapter.
The CIIS strategy-adapter with parameters 
$(K,y,\alpha,l) \in [0,1]\times [0,1] \times ]0, 0.5[ \times \mathds{N}$
is the function that associates to any  $n \in \Nats$ the sequence
$(S^t)^{t \in \mathds{N}}$ defined by: 



 \begin{itemize} 
 \item $K^0 = \textit{bin}(y) \oplus \textit{bin}(K)$: $K^0$ is the real number whose binary decomposition is equal to the bitwise exclusive or (xor)
   between the binary decompositions of $y$ and of  $K$;
 \item $\forall t \leqslant l, K^{t+1} = F(K^t,\alpha)$;
 \item $\forall t \leqslant l, S^t = \left \lfloor n \times K^t \right \rfloor + 1$;
 \item $\forall t > l, S^t = 0$.
 \end{itemize}
where $F$ is the
piecewise linear chaotic map~\cite{Shujun1}, 
recalled in what follows:

\begin{definition}[Piecewise linear chaotic map]
 \label{def:fonction chaotique linéaire par morceaux}
Let $\alpha \in ]0; 0.5[$ be a control parameter. 
The \emph{piecewise linear chaotic map} is the map $F$
defined by: 
 $$
 F(t,\alpha) = \left\{
 \begin{array}{cl} 
 \dfrac{t}{\alpha} & t \in [0; \alpha],\\ 
 \dfrac{t-\alpha}{\frac{1}{2}-\alpha} & t \in [\alpha;\frac{1}{2}],\\ 
 F(1-t,\alpha) & t \in [\frac{1}{2}; 1].\\ 
 \end{array}
 \right. 
 $$
 \end{definition}

Contrary to the logistic map, the use of this piecewise linear chaotic map 
is relevant in cryptographic usages \cite{Arroyo08}.

Parameters of CIIS strategy-adapter will be instantiate as follows: 
$K$ is the secret embedding key, $y$ is the secret message, 
$\alpha$ is the threshold of the piecewise linear chaotic map,
which can be set as $K$ or can act as a second secret key.
Lastly, $l$ is for the iteration number bound:
enlarging its value improve the chaotic behavior of the scheme,
but the time required to achieve the embedding grows too.

Another strategy-adapter is the 
\emph{Chaotic Iterations with Dependent Strategy} (CIDS) 
with parameters $(l,X) \in \mathds{N}\times \mathds{B}^\mathds{N}$, 
which is the function that maps any $ n \in \mathds{N}$ to
the sequence $\left(S^t\right)^{t \in \mathds{N}}$ defined by:
\begin{itemize}
\item $\forall t \leqslant l$, if $t \leqslant l$ and $X^t = 1$, 
  then $S^t=t$, else $S^t=1$;
\item $\forall t > l, S^t = 0$.
\end{itemize}




Let us notice that the terms of $x$ that may be replaced by terms taken
from $y$ are less important than other: they could be changed 
without be perceived as such. More generally, a 
\emph{signification function} 
attaches a weight to each term defining a digital media,
w.r.t. its position $t$:

\begin{definition}[Signification function]
A \emph{signification function} is a real sequence 
$(u^k)^{k \in \Nats}$. % with a limit equal to 0.
\end{definition}








%We first notice that terms of $x$ that may be replaced by terms issued
%from $y$ are less important than other: they could be changed 
%without being perceived as such. More generally, a 
%\emph{signification function} 
%attaches a weight to each terms defining a digital media,
%depending on its position $t$, as follows.

%\begin{definition}[Signification function]
%A \emph{signification function} is a real sequence 
%$(u^k)^{k \in \Nats}$. % with a limit equal to 0.
%\end{definition}

% The convergence to 0 formulates the fact that when we consider just
% one piece of a very large media, the end of this media cannot
% have a great importance according to us.


%\subsubsection{Example}

For instance, let us consider a set of    
grayscale images stored into portable graymap format (P3-PGM):
each pixel ranges between 256 gray levels, \textit{i.e.},
is memorized with eight bits.
In that context, we consider 
$u^k = 8 - (k  \mod  8)$  to be the $k$-th term of a signification function 
$(u^k)^{k \in \Nats}$. 
Intuitively, in each group of eight bits (\textit{i.e.}, for each pixel) 
the first bit has an importance equal to 8, whereas the last bit has an
importance equal to 1. This is compliant with the idea that
changing the first bit affects more the image than changing the last one.





\begin{definition}[Significance of coefficients]\label{def:msc,lsc}
Let $(u^k)^{k \in \Nats}$ be a signification function, 
$m$ and $M$ be two reals s.t. $m < M$. Then 
the \emph{most significant coefficients (MSCs)} of $x$ is the finite 
  vector $u_M$, 
the \emph{least significant coefficients (LSCs)} of $x$ is the 
finite vector $u_m$, and 
the \emph{passive coefficients} of $x$ is the finite vector $u_p$ such that:
\begin{eqnarray*}
  u_M &=& \left( k ~ \big|~ k \in \mathds{N} \textrm{ and } u^k 
    \geqslant M \textrm{ and }  k \le \mid x \mid \right) \\
  u_m &=& \left( k ~ \big|~ k \in \mathds{N} \textrm{ and } u^k 
  \le m \textrm{ and }  k \le \mid x \mid \right) \\
   u_p &=& \left( k ~ \big|~ k \in \mathds{N} \textrm{ and } 
u^k \in ]m;M[ \textrm{ and }  k \le \mid x \mid \right)
\end{eqnarray*}
 \end{definition}

For a given host content $x$,
MSCs are then ranks of $x$  that describe the relevant part
of the image, whereas LSCs translate its less significant parts.
We are then ready to decompose an host $x$ into its coefficients and 
then to recompose it. Next definitions formalize these two steps. 

\begin{definition}[Decomposition function]
Let $(u^k)^{k \in \Nats}$ be a signification function, 
$\mathfrak{B}$ the set of finite binary sequences,
$\mathfrak{N}$ the set of finite integer sequences, 
$m$ and $M$ be two reals s.t. $m < M$.  
Any host $x$ can be decomposed into 
\[
(u_M,u_m,u_p,\phi_{M},\phi_{m},\phi_{p})
\in
\mathfrak{N} \times 
\mathfrak{N} \times 
\mathfrak{N} \times 
\mathfrak{B} \times 
\mathfrak{B} \times 
\mathfrak{B} 
\]
where
\begin{itemize}
\item $u_M$, $u_m$, and $u_p$ are coefficients defined in Definition  
\ref{def:msc,lsc};
\item $\phi_{M} = \left( x^{u^1_M}, x^{u^2_M}, \ldots,x^{u^{|u_M|}_M}\right)$;
 \item $\phi_{m} = \left( x^{u^1_m}, x^{u^2_m}, \ldots,x^{u^{|u_m|}_m} \right)$;
 \item $\phi_{p} =\left( x^{u^1_p}, x^{u^2_p}, \ldots,x^{u^{|u_p|}_p}\right) $.
 \end{itemize}
The function that associates the decomposed host to any digital host is 
the \emph{decomposition function}. It is 
further referred as $\textit{dec}(u,m,M)$ since it is parametrized by 
$u$, $m$, and $M$. Notice that $u$ is a shortcut for $(u^k)^{k \in \Nats}$.
\end{definition} 


\begin{definition}[Recomposition]
Let 
$(u_M,u_m,u_p,\phi_{M},\phi_{m},\phi_{p}) \in 
\mathfrak{N} \times 
\mathfrak{N} \times 
\mathfrak{N} \times 
\mathfrak{B} \times 
\mathfrak{B} \times 
\mathfrak{B} 
$ s.t.
\begin{itemize}
\item the sets of elements in $u_M$, elements in $u_m$, and 
elements in $u_p$ are a partition of $\llbracket 1, n\rrbracket$;
\item $|u_M| = |\varphi_M|$, $|u_m| = |\varphi_m|$, and $|u_p| = |\varphi_p|$.  
\end{itemize}
One can associate the vector 
\[
x = 
\sum_{i=1}^{|u_M|} \varphi^i_M . e_{{u^i_M}} +  
\sum_{i=1}^{|u_m|} \varphi^i_m .e_{{u^i_m}} +  
\sum_{i=1}^{|u_p|} \varphi^i_p. e_{{u^i_p}} 
\]
\noindent where 
%$e_i$ is the sequence whose $j-$th term is equal to $\overline{\Delta(i,j)}$, \emph{i.e.}, 
$(e_i)_{i \in \mathds{N}}$ is the usual basis of the $\mathds{R}-$vectorial space $\left(\mathds{R}^\mathds{N}, +, .\right)$ (that is to say, $e_i^j = \delta_{ij}$, where $\delta_{ij}$ is the Kronecker symbol).
The function that associates $x$ to any 
$(u_M,u_m,u_p,\phi_{M},\phi_{m},\phi_{p})$ following the above constraints 
is called the \emph{recomposition function}.
\end{definition}

The embedding consists in the replacement of the values of 
$\phi_{m}$ of $x$'s LSCs  by $y$. 
It then composes the two decomposition and
recomposition functions seen previously. More formally:


\begin{definition}[Embedding media]
Let $\textit{dec}(u,m,M)$ be a decomposition function,
$x$ be a host content,
$(u_M,u_m,u_p,\phi_{M},\phi_{m},\phi_{p})$ be its image by $\textit{dec}(u,m,M)$, 
and $y$ be a digital media of size $|u_m|$.
The digital media $z$ resulting on the embedding of $y$ into $x$ is 
% the
% result of the \emph{embedding} of $y$ in $x$ if 
%  $$
%  \forall n \in \llbracket1, |x|\rrbracket , z^n = \left\{
%  \begin{array}{ll}
%  x^n & \textrm{if } \phi^n_m > m,\\
%  y^n & \textrm{else.}
%  \end{array}
%  \right.
%  $$
%  
% In other words, $z$ is
the image of $(u_M,u_m,u_p,\phi_{M},y,\phi_{p})$
by  the recomposition function $\textit{rec}$.
\end{definition}

Let us then define the dhCI information hiding scheme
presented in~\cite{gfb10:ip}:

\begin{definition}[Data hiding dhCI]
 \label{def:dhCI}
Let $\textit{dec}(u,m,M)$ be a decomposition function,
$f$ be a mode, 
$\mathcal{S}$ be a strategy adapter,
$x$ be an host content,\linebreak
$(u_M,u_m,u_p,\phi_{M},\phi_{m},\phi_{p})$ 
be its image by $\textit{dec}(u,m,M)$,
$q$ be a positive natural number,  
and $y$ be a digital media of size $l=|u_m|$.


The dhCI dissimulation  maps any
$(x,y)$  to the digital media $z$ resulting on the embedding of
$\hat{y}$ into $x$, s.t.

\begin{itemize}
\item we instantiate the mode $f$ with parameter $l=|u_m|$, leading to 
  the function $f_{l}:\Bool^{l} \rightarrow \Bool^{l}$;
\item we instantiate the strategy adapter $\mathcal{S}$ 
with parameter $y$ (and possibly some other ones);
this instantiation leads to the strategy $S_y \in \llbracket 1;l\rrbracket ^{\Nats}$.

\item we iterate $G_{f_l}$ with initial configuration $(S_y,\phi_{m})$;
\item $\hat{y}$ is finally the $q$-th term of these iterations.
\end{itemize}
\end{definition}


To summarize, iterations are realized on the LSCs of the
host content
(the mode gives the iterate function,  
the strategy-adapter gives its strategy), 
and the last computed configuration is re-injected into the host content, 
in place of the former LSCs.



%\begin{definition}[Significance of coefficients]\label{def:msc,lsc}
%Let $(u^k)^{k \in \Nats}$ be a signification function, 
%$m$ and $M$ be two reals s.t. $m < M$. Then 
%the \emph{most significant coefficients (MSCs)} of $x$ is the finite 
%  vector $u_M$, 
%the \emph{least significant coefficients (LSCs)} of $x$ is the 
%finite vector $u_m$, and 
%the \emph{passive coefficients} of $x$ is the finite vector $u_p$ such that:
%\begin{eqnarray*}
%  u_M &=& \left( k ~ \big|~ k \in \mathds{N} \textrm{ and } u^k 
%    \geqslant M \textrm{ and }  k \le \mid x \mid \right) \\
%  u_m &=& \left( k ~ \big|~ k \in \mathds{N} \textrm{ and } u^k 
%  \le m \textrm{ and }  k \le \mid x \mid \right) \\
%   u_p &=& \left( k ~ \big|~ k \in \mathds{N} \textrm{ and } 
%u^k \in ]m;M[ \textrm{ and }  k \le \mid x \mid \right)
%\end{eqnarray*}
% \end{definition}

%For a given host content $x$,
%MSCs are then ranks of $x$  that describe the relevant part
%of the image, whereas LSCs translate its less significant parts.
%We are then ready to decompose an host $x$ into its coefficients and 
%then to recompose it. Next definitions formalize these two steps. 

%\begin{definition}[Decomposition function]
%Let $(u^k)^{k \in \Nats}$ be a signification function, 
%$\mathfrak{B}$ the set of finite binary sequences,
%$\mathfrak{N}$ the set of finite integer sequences, 
%$m$ and $M$ be two reals s.t. $m < M$.  
%Any host $x$ may be decomposed into 
%$$
%(u_M,u_m,u_p,\phi_{M},\phi_{m},\phi_{p})
%\in
%\mathfrak{N} \times 
%\mathfrak{N} \times 
%\mathfrak{N} \times 
%\mathfrak{B} \times 
%\mathfrak{B} \times 
%\mathfrak{B} 
%$$
%where
%\begin{itemize}
%\item $u_M$, $u_m$, and $u_p$ are coefficients defined in Definition  
%\ref{def:msc,lsc};
%\item $\phi_{M} = \left( x^{u^1_M}, x^{u^2_M}, \ldots,x^{u^{|u_M|}_M}\right)$;
% \item $\phi_{m} = \left( x^{u^1_m}, x^{u^2_m}, \ldots,x^{u^{|u_m|}_m} \right)$;
% \item $\phi_{p} =\left( x^{u^1_p}, x^{u^2_p}, \ldots,x^{u^{|u_p|}_p}\right) $.
% \end{itemize}
%The function that associates the decomposed host to any digital host is 
%the \emph{decomposition function}. It is 
%further referred as $\textit{dec}(u,m,M)$ since it is parametrized by 
%$u$, $m$, and $M$. Notice that $u$ is a shortcut for $(u^k)^{k \in \Nats}$.
%\end{definition} 


%\begin{definition}[Recomposition]
%Let 
%$(u_M,u_m,u_p,\phi_{M},\phi_{m},\phi_{p}) \in 
%\mathfrak{N} \times 
%\mathfrak{N} \times 
%\mathfrak{N} \times 
%\mathfrak{B} \times 
%\mathfrak{B} \times 
%\mathfrak{B} 
%$ s.t.
%\begin{itemize}
%\item the sets of elements in $u_M$, elements in $u_m$, and 
%elements in $u_p$ are a partition of $\llbracket 1, n\rrbracket$;
%\item $|u_M| = |\varphi_M|$, $|u_m| = |\varphi_m|$, and $|u_p| = |\varphi_p|$.  
%\end{itemize}
%One may associate the vector 
%$$x = 
%\sum_{i=1}^{|u_M|} \varphi^i_M . e_{{u^i_M}} +  
%\sum_{i=1}^{|u_m|} \varphi^i_m .e_{{u^i_m}} +  
%\sum_{i=1}^{|u_p|} \varphi^i_p. e_{{u^i_p}} 
%$$
%\noindent where $e_i$ is the sequence whose $j-$th term is equal to $\overline{\Delta(i,j)}$, \emph{i.e.}, $(e_i)_{i \in \mathds{N}}$ is the usual basis of the $\mathds{R}-$vectorial space $\left(\mathds{R}^\mathds{N}, +, .\right)$.
%The function that associates $x$ to any 
%$(u_M,u_m,u_p,\phi_{M},\phi_{m},\phi_{p})$ following the above constraints 
%is called the \emph{recomposition function}.
%\end{definition}

%The embedding consists to the replacement of the values of 
%$\phi_{m}$ of $x$'s LSCs  by $y$. 
%It then composes the two decomposition and
%recomposition functions seen previously. More formally:


%\begin{definition}[Embedding digital media]
%Let $\textit{dec}(u,m,M)$ be a decomposition function,
%$x$ be a host content,
%$(u_M,u_m,u_p,\phi_{M},\phi_{m},\phi_{p})$ be its image by $\textit{dec}(u,m,M)$,
%and $y$ be a digital media of size $|u_m|$.
%The digital media $z$ resulting on the embedding of $y$ into $x$ is 
%% the
%% result of the \emph{embedding} of $y$ in $x$ if 
%%  $$
%%  \forall n \in \llbracket1, |x|\rrbracket , z^n = \left\{
%%  \begin{array}{ll}
%%  x^n & \textrm{if } \phi^n_m > m,\\
%%  y^n & \textrm{else.}
%%  \end{array}
%%  \right.
%%  $$
%%  
%% In other words, $z$ is
%the image of $(u_M,u_m,u_p,\phi_{M},y,\phi_{p})$
%by  the recomposition function $\textit{rec}$.
%\end{definition}

%We can now define the information hiding scheme called \emph{dhCI}:

%\begin{definition}[Data hiding dhCI]
% \label{def:dhCI}
%Let $\textit{dec}(u,m,M)$ be a decomposition function,
%$f$ be a mode, 
%$\mathcal{S}$ be a strategy adapter,
%$x$ be an host content,\linebreak
%$(u_M,u_m,u_p,\phi_{M},\phi_{m},\phi_{p})$ be its image by $\textit{dec}(u,m,M)$,  
%and $y$ be a digital media of size $l=|u_m|$.


%The \emph{dhCI dissimulation} is the application that maps any
%$(x,y)$  to the digital media $z$ resulting on the embedding of
%$\hat{y}$ into $x$, s.t.

%\begin{itemize}
%\item We instantiate the mode $f$ with parameter $l=|u_m|$, leading to 
%  the function $f_{l}:\Bool^{l} \rightarrow \Bool^{l}$.
%\item We instantiate the strategy adapter $\mathcal{S}$ 
%with parameter $y$ (and some other ones eventually). 
%This instantiation leads to the strategy $S_y \in \llbracket 1;l\rrbracket ^{\Nats}$.

%\item We iterate $G_{f_l}$ with initial configuration $(S_y,\phi_{m})$.
%\item $\hat{y}$ is finally the $l$-th term of these iterations.
%\end{itemize}
%\end{definition}


%To summarize, some iterations are realized on the LSCs of the
%host content
%(the mode gives the iterate function,  
%the strategy-adapter gives its strategy), 
%and the last computed state is re-injected into the host content, 
%in place of the former LSCs.






Notice that in order to preserve the unpredictable behavior of the system, 
the size of the digital medias is not fixed.
This approach is thus self adapted to any media, and more particularly to
any size of LSCs. 
However this flexibility enlarges the complexity of the presentation: 
we had to give Definitions~\ref{def:mode} and~\ref{def:strategy-adapter} 
respectively of mode and strategy adapter.

\begin{figure}[ht]
\centering
%\includegraphics[width=8.5cm]{organigramme2.pdf}
\includegraphics[width=8.5cm]{organigramme2.eps}
\caption{The dhCI dissimulation scheme}
\label{fig:organigramme}
\end{figure}


Next section shows how to check whether a media contains a watermark.


==> wmdecoding.tex <==

Let us firstly show how to formally check whether a given digital media $z$ 
results from the dissimulation of $y$ into the digital media $x$. 



\begin{definition}[Watermarked content]
Let $\textit{dec}(u,m,M)$ be a decomposition function,
$f$ be a mode, 
$\mathcal{S}$ be a strategy adapter, 
$q$ be a positive natural number,  
$y$ be a digital media, and 
$(u_M,u_m,u_p,\phi_{M},\phi_{m},\phi_{p})$ be the 
image by $\textit{dec}(u,m,M)$  of  a digital media $x$. 
Then $z$ is \emph{watermarked} with $y$ if
the image by $\textit{dec}(u,m,M)$ of $z$ is 
$(u_M,u_m,u_p,\phi_{M},\hat{y},\phi_{p})$, where 
$\hat{y}$ is the right member of $G_{f_l}^q(S_y,\phi_{m})$.
\end{definition}


Various decision strategies are obviously  possible to determine whether a given
image $z$ is watermarked or not, depending  on the eventuality
that the considered image may have  been attacked.
For example, a  similarity percentage between $x$
and  $z$ can  be  computed and compared  to a  given
threshold. Other  possibilities are the use of  ROC curves or
the definition of a null hypothesis problem.





%\begin{definition}[Marked content]
%Let $\textit{dec}(u,m,M)$ be a decomposition function,
%$f$ be a mode, 
%$\mathcal{S}$ be a strategy adapter, and  
%$y$ be a digital media, \linebreak
%$(u_M,u_m,u_p,\phi_{M},\phi_{m},\phi_{p})$ be the 
%image by $\textit{dec}(u,m,M)$  of  a digital media $x$. 
%Then $z$ is \emph{marked} with $y$ if
%the image by $\textit{dec}(u,m,M)$ of $z$ is 
%$(u_M,u_m,u_p,\phi_{M},\hat{y},\phi_{p})$.
%\end{definition}


%Various decision strategies are obviously  possible to determine whether a given
%image $z$ is  marked or not, depending  on the eventuality
%that the considered image may have  been attacked.
%For example, a  similarity percentage between $x$
%and  $z$ can  be  computed, and  the result  can  be compared  to a  given
%threshold. Other  possibilities are the use of  ROC curves or
%the definition of a null hypothesis problem.

% Thus only a  binary information can finally be embedded into  a given host, when
% using  the  dhCI dissimulation  algorithm:  hidden  message  $y$ is  more
% related  to a  private  embedding  key. Moreover,  this  data hiding scheme  is
% non-blind  as  the  original host  is  required  to  extract the  binary  hidden
% information.  These two  strong requirements  can lead  to the  belief  that the
% dhCI dissimulation is finally not  really helpful in most situations that
% occur in information hiding.

% However, as stated in the
% introduction, such requirements are not so strong 
% as it could primarily appear:  it allows to prove that we
% are the  author of  a document sent  through the  Internet; we thus can
% store the original document and send the  stego content.
% Secondly, Alice and Bob can
% establish an hidden channel into a  streaming video: Alice and Bob both have the
% same movie, and  Alice will hide information into 
% the frame number $k$  iff the binary digit
% number $k$ of its hidden message is  1. Thirdly, based on a similar idea, a same
% given image can be marked  several times by using various secret parameters
% owned both by Alice and Bob. Thus more than one bit can be embedded into a given
% image  by using  dhCI  dissimulation. Lastly,  non-blind watermarking  is
% useful in  network's anonymity and intrusion  detection \cite{Houmansadr09}, and
% to protect digital data sending through the Internet \cite{P1150442004}.

%  Additionally, this scheme can be adapted to
% situations where  security is not a  strong requirement, as  follows. Instead of
% realizing  chaotic iterations  on  LSCs, it  is  also possible  to replace  bits
% selected  by  the  chaotic strategy  with  those  of  the hidden  message.  This
% replacement (in place of the switch)  leads to the ability to extract the hidden
% bits, but the security of the scheme is consequently reduced to the sole chaotic
% selection of LSCs.

The next section recalls some security properties and shows how the 
\emph{dhCI dissimulation} algorithm verifies them.

